The formation of an eccentric gap in a gas disk by a planet in an eccentric orbit

We investigate the effect of a planet on an eccentric orbit on a two dimensional low mass gaseous disk. At a planet eccentricity above the planet's Hill radius divided by its semi-major axis, we find that the disk morphology differs from that exhibited by a disk containing a planet in a circular orbit. An eccentric gap is created with eccentricity that can exceed the planet's eccentricity and precesses with respect to the planet's orbit. We find that a more massive planet is required to open a gap when the planet is on an eccentric orbit. We attribute this behavior to spiral density waves excited at corotation resonances that increase the disk's eccentricity and exert a torque opposite in sign to that exerted by the Lindblad resonances. The reduced torque makes it more difficult for waves driven by the planet to overcome viscous inflow in the disk. Spectral energy distributions of transitional disks may reveal the presence of an eccentric planet if they are matched by an inner edge comprising a range of temperatures set by the semi-major axis and eccentricity of the hole.

==> Makefile <==
rootDoc = eccgaps

bibliogs = general.bib

sources = intro.tex\
          numeric.tex\
          circular.tex\
          eccentric.tex\
          newcriterion.tex\
          discuss.tex\
          summary.tex

others = commands.tex planetcommands.tex

$(rootDoc).dvi: $(rootDoc).tex $(sources) $(bibliogs) $(others)
	latex   $(rootDoc)
	bibtex  $(rootDoc)
	latex   $(rootDoc)
	latex   $(rootDoc)

display: $(rootDoc).dvi
	latex $(rootDoc)
	xdvi -geometry 920x900 -s 8 $(rootDoc)

postscript: $(rootDoc).dvi
	latex $(rootDoc)
	dvips -o $(rootDoc).ps $(rootDoc).dvi

pdf: $(rootDoc).dvi
	pdflatex $(rootDoc)

clean:
	-rm *.dvi
	-rm *.aux
	-rm *.log
	-rm *.bbl
	-rm *.blg
	-rm *~
	-rm $(rootDoc).ps
	-rm $(rootDoc).pdf


tarball:
	make clean
	tar --exclude CVS -cvzhf ../paper.tgz ../SummerPaper/
